Universal Paralinguistic Speech Representations Using Self-Supervised Conformers

Many speech applications require understanding aspects beyond the words being spoken, such as recognizing emotion, detecting whether the speaker is wearing a mask, or distinguishing real from synthetic speech. In this work, we introduce a new state-of-the-art paralinguistic representation derived from large-scale, fully self-supervised training of a 600M+ parameter Conformer-based architecture. We benchmark on a diverse set of speech tasks and demonstrate that simple linear classifiers trained on top of our time-averaged representation outperform nearly all previous results, in some cases by large margins. Our analyses of context-window size demonstrate that, surprisingly, 2 second context-windows achieve 96\% the performance of the Conformers that use the full long-term context on 7 out of 9 tasks. Furthermore, while the best per-task representations are extracted internally in the network, stable performance across several layers allows a single universal representation to reach near optimal performance on all tasks.

==> table_results_v0.tex <==
\begin{centering}
\begin{table*}[t]
\vspace{-0.2cm}
\captionsetup{size=footnotesize}
%\caption{Accuracies (\%) for NOSS tasks. }
\caption{Test performance on the NOSS Benchmark and extended tasks. ``Prev SoTA" are arbitrarily complicated models, but \textbf{all other rows are linear models on time-averaged input}.
$^\dagger$We use a filtered subset of Voxceleb1 according to YouTube’s privacy guidelines. We omit previous SoTA results on this dataset, since they used the entire dataset.
$^\ddagger$The Masked Speech task performance is reported using unweighted average recall~\cite{compare2020} instead of accuracy. Also, test set labels are not available, so we report accuracy on the eval set. 
$^{**}$ASVSpoof uses equal error rate~\cite{asvspoof}.
$^{\#}$Euphonia is the only non-public dataset. We exclude it from aggregate scores.
$^{\dagger\dagger}$SAVEE is included in the table but not aggregate score, since its less than 1/10th the size of the next smallest dataset and results have high variance.
$^*$Audio and visual features used in previous SoTA.
$^{+}$Prev SOTA performed cross-fold validation. We hold out speakers M05 and F05 as test.
$^{\small++}$YAMNet uses layer 10, as in~\cite{trill}.
$^\mathsection$Best per-task results are compute by taking the model/layer with the best results of the dev set, and reporting those results on the test set. If the dev set performance is better but the test results are worse, ``Best per-task" can be worse than ``Best overall".
}\label{tab:results}

\footnotesize
\centering
\begin{tabular}{@{} l|ccccccccc @{}}
\toprule[2pt]
Model & 
Voxceleb1$^\dagger$ & 
Voxforge & 
\begin{tabular}{@{}c@{}}Speech \\ Commands\end{tabular}   &  
\begin{tabular}{@{}c@{}}Masked \\ Speech$^\ddagger$\end{tabular}  & 
\begin{tabular}{@{}c@{}}ASVSpoof\\ 2019$^{**}$\end{tabular} & 
Euphonia$^{\#}$ &
CREMA-D &
IEMOCAP &
SAVEE$^{\dagger\dagger}$
\\
\toprule[2pt]
\textbf{Prev SoTA}
& - 
& 95.4 \cite{sarthak2019spoken} 
& \textbf{97.9}~\cite{speech_commandssota} 
& 73.0~\cite{Szep2020} 
& 5.11~\cite{superb} 
& 45.9~\cite{asremb}
& 74.0$^*$ \cite{ghaleb2019} 
& 67.6$^{+}$~\cite{superb} 
& 84.0$^*$~\cite{savee} 
%& ?~\cite{asremb}  
\\
\midrule
\textbf{Baselines} \\
% voxceleb voxforge speechcommands maskchallenge asvspoof euphonia cremad iemocap savee
\quad YAMNet$^{\small++}$ \cite{trill} 
& 10.9 & 79.8 & 78.5 & 59.7 & 9.23 & 43.0 & 66.4 & 57.5 & 69.2  \\
\quad TRILL \cite{trill}
& 12.6 & 84.5 & 77.6 & 65.2 & 7.46 & 48.1 & 65.7 & 54.3 & 65.0\\
\quad FRILL \cite{frill}   
& 13.8 & 78.8 & 74.4 & 67.2 & 7.45 & 46.6 & 71.3 & 57.6 & 63.3\\
\quad COLA \cite{cola}
& 11.7 & 71.0 & 60.6 & 65.0 & 4.58 & 47.6 & 69.3 & 63.9 & 59.2 \\
\quad ASR Emb \cite{asremb}
& 5.2 & 98.9 & 96.1  & 54.4 & 11.2 & \textbf{54.5} & 71.8 & 65.4 & 85.0\\
\midrule
\textbf{Conformers} \\
% voxceleb voxforge speechcommands maskchallenge asvspoof euphonia cremad iemocap savee 
\quad 
Best per-task$^\mathsection$ &
\textbf{53.5} & \textbf{99.8} & 97.5  & \textbf{74.2} & \textbf{2.5} & 53.6 & 87.2 & \textbf{79.2} & \textbf{92.5} \\
\quad  (model, layer \#) &
(XXL-YT, 25) & (G-YT, 19) & (CAP, 16) & (XL-LL RA, 5) & (CAP, 12) & (CAP, 13) & (G, 26) & (CAP, 15) & (CAP, 15) \\
\midrule
\quad 
\begin{tabular}{@{}c@{}}Best CAP per\\ task (layer \#)\end{tabular} &
50.3 (11) & 99.7 (14) & 97.5 (16) & 73.4 (10) & \textbf{2.5} (12)  & 53.6 (13) & \textbf{88.2}$^\mathsection$ (12) & \textbf{79.2} (15) & 92.5 (15) \\
\midrule
\quad 
\begin{tabular}{@{}c@{}}Best single\\ layer (CAP12)\end{tabular} &
51.0$^\mathsection$ & 99.7 & 97.0 & 68.9 & \textbf{2.5} & 51.5 & \textbf{88.2}$^\mathsection$ & 75.0 & 81.7\\
\bottomrule
\end{tabular}
\vspace{-3mm}
\end{table*}
\end{centering}

==> unused_discussion.tex <==
% DISCUSSION SECTION IS NOW OMITTED, WITH FIG AND FIRST PARAGRAPH MOVED TO EXPERIMENTS
%\begin{figure}[t]
%{\centering
%  \includegraphics[width=0.7\columnwidth]{images/comparison.pdf}\hspace{0.2cm}
%  \vspace{-4mm}
%  \captionsetup{size=footnotesize}
%  \caption{$P( \mbox{Model Y is correct} | \mbox{Model X and Y disagree}) $. Each square is the probability that Model Y correctly %predicts an example given that Model X and Model Y disagree on the prediction, averaged over all examples in all downstream %datasets.}\label{fig:comparison}}
%  \vspace{-3mm}
%\end{figure}

%\textbf{CAP12 is strictly better than other representations}: Since aggregate performance ignores patterns of errors, we investigate the agreement between predictions made from different embeddings on a per-example basis to determine whether CAP12 is strictly better than alternatives.  We see in Figure~\ref{fig:comparison} that when CAP12 and other embeddings disagree, CAP12 is correct on 43\% to 75\% of the examples. When they disagree, other embeddings are correct on only 15\%-40\% of the examples. This shows that with the possible exception of the ASR Embedding, it is uncommon for other embeddings to be correct with CAP12 is wrong.

%\textbf{Our self-supervised contrastive loss is not optimized for paralinguistic speech:} If the Wav2Vec 2.0 loss was aligned with the goal of paralinguistic analisys, we would expect the best-performing layer to be at or close to the final layer. Instead, Figures~\ref{fig:context} and~\ref{fig:layerwise_analysis} show that the best representation for paralinguistic tasks is close to the middle of the Conformer models, for all context-window sizes, all architectures, and all datasets.  This indicates that the self-supervised loss function might be improved for paralinguistics, which could lead to even better representations of speech.
